Casting the Net! Revisiting MasterFace Impersonation Attacks

Impersonation is a fundamental security threat in face recognition systems (FRSs). While the security of FRSs has been challenged by various attack vectors, under realistic adversarial capabilities, e.g., a limited number of decision-only authentication trials and no internal system knowledge, most attack techniques become infeasible. As a result, impersonation by zero-effort impostors, characterized by false match rate (FMR), is commonly regarded as a standalone baseline. A few years ago, impersonation attacks based on MasterFaces emerged as a notable security threat that could break the barrier of the FMR-based baseline under such realistic constraints. However, they were believed not to yield impersonation above the standard FMR in modern FRSs, as discussed by multiple follow-up studies. In this paper, we demonstrate that even legitimate access to public commercial APIs allows an adversary to amplify impersonation rates through MasterFaces, resulting in a non-trivial impersonation attack beyond FMR on downstream applications built on top of these APIs. We observe that several real-world FRS deployments are implemented using commercial APIs, and that the backend service provider is publicly disclosed or trivially inferable. As a result, the adversary can purchase these pay-as-you-go API services without requiring any additional privilege over the target FRS. From this observation, we formalize the MasterFaces attack as a maximum coverage problem over the biometric representation space, which we call a NET, and show that the adversary can construct an API-tailored NET by leveraging the geometric structure of the representation space. We demonstrate that our attack amplifies the impersonation rates of several open-source and commercial API-based FRSs by up to 9.5$\times$ within at most 30 authentication trials, compared to those expected from the standard FMR.

==> figs/OldData.tex <==
%
%
%
%
% \begin{table*}[ht]
% \centering
% \caption{Comparison of EER and minDCF}
% \label{tab:results}
% \begin{tabular}{|c|c|c|cc|cc|cc|}
% \hline
% \multirow{2}{*}{Q} & \multirow{2}{*}{Ratio} & \multirow{2}{*}{$\tau$} 
% & \multicolumn{2}{c|}{Center} 
% & \multicolumn{2}{c|}{Image} 
% & \multicolumn{2}{c|}{Exact Inv. Img} \\
% \cline{4-9}
% & & & EER(\%) & minDCF(\%) & EER(\%) & minDCF(\%) & EER(\%) & minDCF(\%) \\
% \hline
% 5 & 20 & 0.5 & 45.28\% & 21.26\% & 12.02\% & 1.04\% & 23.11\% & 6.12\% \\
% 5 & 15 & 0.6 & 40.29\% & 18.18\% & 9.43\% & 2.38\% & 21.96\% & 6.99\% \\
% 5 & 20 & 0.4 & 48.49\% & 16.55\% & 8.24\% & 0.70\% & 18.67\% & 4.78\% \\
% 5 & 20 & 0.6 & 41.36\% & 19.12\% & 7.35\% & 0.59\% & 21.09\% & 6.31\% \\
% 5 & 25 & 0.6 & 37.68\% & 17.44\% & 7.99\% & 0.96\% & 19.94\% & 5.82\% \\
% \hline
% 10 & 10 & 0.5 & 62.55\% & 29.12\% & 16.69\% & 1.25\% & 33.37\% & 9.28\% \\
% 10 & 5 & 0.5 & 64.12\% & 23.41\% & 11.72\% & 2.49\% & 27.38\% & 3.08\% \\
% 10 & 15 & 0.6 & 52.70\% & 27.91\% & 13.32\% & 1.70\% & 28.04\% & 8.16\% \\
% 10 & 10 & 0.4 & 62.17\% & 21.47\% & 10.49\% & 0.91\% & 25.85\% & 7.75\% \\
% 10 & 10 & 0.6 & 53.06\% & 23.60\% & 11.96\% & 0.87\% & 26.74\% & 7.14\% \\
% \hline
% 20 & 5 & 0.5 & 78.82\% & 36.62\% & 17.31\% & 1.30\% & 43.05\% & 9.83\% \\
% 20 & 30 & 0.5 & 72.18\% & 29.44\% & 15.99\% & 2.53\% & 36.62\% & 7.03\% \\
% 20 & 5 & 0.6 & 62.74\% & 32.41\% & 18.95\% & 2.10\% & 35.81\% & 9.45\% \\
% 20 & 25 & 0.5 & 73.24\% & 27.29\% & 14.87\% & 1.49\% & 34.49\% & 7.35\% \\
% 20 & 20 & 0.5 & 72.32\% & 28.80\% & 13.23\% & 2.15\% & 33.60\% & 7.22\% \\
% \hline
% 30 & 30 & 0.5 & 79.72\% & 35.66\% & 20.56\% & 4.91\% & 42.16\% & 10.09\% \\
% 30 & 5 & 0.5 & 78.97\% & 36.75\% & 20.37\% & 1.78\% & 42.93\% & 8.56\% \\
% 30 & 20 & 0.5 & 77.27\% & 31.84\% & 15.74\% & 3.06\% & 40.55\% & 6.63\% \\
% 30 & 15 & 0.5 & 75.15\% & 31.44\% & 14.02\% & 2.63\% & 39.23\% & 7.39\% \\
% 30 & 5 & 0.6 & 65.19\% & 35.71\% & 21.24\% & 2.21\% & 36.32\% & 8.98\% \\
% \hline
% 50 & 5 & 0.5 & 88.95\% & 39.38\% & 19.29\% & 3.02\% & 49.70\% & 9.77\% \\
% 50 & 25 & 0.6 & 73.64\% & 38.49\% & 27.57\% & 5.73\% & 45.79\% & 14.36\% \\
% 50 & 10 & 0.5 & 88.36\% & 36.58\% & 21.26\% & 2.19\% & 47.01\% & 9.39\% \\
% 50 & 25 & 0.5 & 82.43\% & 35.20\% & 20.73\% & 3.80\% & 44.73\% & 10.81\% \\
% 50 & 20 & 0.6 & 73.83\% & 36.72\% & 23.90\% & 5.90\% & 43.03\% & 13.00\% \\
% \hline
% 100 & 10 & 0.5 & 93.12\% & 51.68\% & 30.73\% & 5.12\% & 64.25\% & 14.74\% \\
% 100 & 5 & 0.5 & 94.52\% & 47.18\% & 28.91\% & 4.57\% & 60.64\% & 14.46\% \\
% 100 & 10 & 0.6 & 87.49\% & 46.50\% & 31.78\% & 6.88\% & 55.27\% & 18.63\% \\
% 100 & 20 & 0.5 & 91.91\% & 48.68\% & 28.55\% & 1.38\% & 61.38\% & 12.02\% \\
% 100 & 25 & 0.5 & 88.66\% & 46.09\% & 32.71\% & 4.01\% & 59.15\% & 12.72\% \\
% \hline
% \end{tabular}
% \end{table*}


% \begin{table*}
%     \begin{tabular}{|c|c|c|cc|cc|cc|}
% \hline
% \multirow{2}{*}{Q} & \multirow{2}{*}{Ratio} & \multirow{2}{*}{$\tau$} 
% & \multicolumn{2}{c|}{Center} 
% & \multicolumn{2}{c|}{Image} 
% & \multicolumn{2}{c|}{Exact Inv. Img} \\
% \cline{4-9}
% & & & EER(\%) & minDCF(\%) & EER(\%) & minDCF(\%) & EER(\%) & minDCF(\%) \\
% \hline
% 5 & 15 & 0.6 & 8.24\% & 0.28\% & 7.48\% & 0.13\% \\
% 5 & 15 & 0.4 & 8.54\% & 0.45\% & 6.18\% & 0.70\% \\
% 5 & 30 & 0.3 & 7.43\% & 0.64\% & 7.26\% & 0.21\% \\
% 5 & 30 & 0.5 & 6.95\% & 0.53\% & 7.67\% & 0.23\% \\
% 5 & 30 & 0.6 & 9.43\% & 0.55\% & 4.69\% & 0.08\% \\
% \hline
% 10 & 15 & 0.6 & 11.96\% & 0.59\% & 15.27\% & 0.74\% \\
% 10 & 20 & 0.5 & 10.56\% & 2.06\% & 8.67\% & 1.47\% \\
% 10 & 30 & 0.3 & 9.32\% & 0.55\% & 11.70\% & 0.59\% \\
% 10 & 25 & 0.5 & 9.58\% & 0.68\% & 9.15\% & 0.57\% \\
% 10 & 15 & 0.1 & 8.92\% & 0.72\% & 8.92\% & 0.40\% \\
% \hline
% 20 & 25 & 0.5 & 20.62\% & 2.06\% & 14.17\% & 1.08\% \\
% 20 & 30 & 0.5 & 18.88\% & 1.95\% & 16.65\% & 0.38\% \\
% 20 & 25 & 0.2 & 17.82\% & 1.68\% & 14.40\% & 1.51\% \\
% 20 & 20 & 0.5 & 16.31\% & 1.17\% & 15.40\% & 0.62\% \\
% 20 & 20 & 0.4 & 17.33\% & 1.25\% & 14.08\% & 0.51\% \\
% \hline
% 30 & 30 & 0.5 & 24.30\% & 2.53\% & 23.00\% & 1.32\% \\
% 30 & 25 & 0.4 & 23.13\% & 2.44\% & 18.88\% & 0.64\% \\
% 30 & 15 & 0.1 & 20.69\% & 1.04\% & 18.97\% & 0.76\% \\
% 30 & 20 & 0.5 & 19.90\% & 1.70\% & 17.25\% & 1.44\% \\
% 30 & 20 & 0.3 & 18.69\% & 1.21\% & 18.76\% & 0.83\% \\
% \hline
% 50 & 15 & 0.4 & 26.13\% & 2.02\% & 25.91\% & 2.53\% \\
% 50 & 10 & 0.1 & 24.38\% & 1.27\% & 28.16\% & 1.95\% \\
% 50 & 10 & 0.5 & 26.23\% & 2.08\% & 23.77\% & 1.27\% \\
% 50 & 25 & 0.6 & 27.19\% & 2.08\% & 23.36\% & 0.53\% \\
% 50 & 25 & 0.5 & 26.06\% & 1.42\% & 23.60\% & 1.19\% \\
% \hline
% 100 & 10 & 0.6 & 41.65\% & 3.91\% & 36.64\% & 1.89\% \\
% 100 & 10 & 0.5 & 41.74\% & 3.59\% & 33.64\% & 1.85\% \\
% 100 & 25 & 0.5 & 36.81\% & 4.18\% & 33.41\% & 2.32\% \\
% 100 & 25 & 0.6 & 33.98\% & 3.61\% & 34.26\% & 2.34\% \\
% 100 & 30 & 0.5 & 32.77\% & 3.84\% & 34.30\% & 1.55\% \\
% \hline
% \end{tabular}
% \end{table*}


==> figs/Tab1.tex <==
\begin{table*}[t]
    \caption{Comparison between the proposed attack and existing ones in terms of adversarial goal and capability. 
    Capabilities colored in \textbf{\textcolor{red}{red}} do not hold for our realistic adversarial model (i) direct score query to the target identity is not permitted, and (ii) target information is unknown.
    }
    \vspace{-10pt}
    \centering
    \begin{tabular}{c|c|c|c|c|c}
        \hline 
        \multirow{2}{*}{Attacks} & \multirow{2}{*}{Adversarial Goal} & \multicolumn{3}{c|}{Adversarial Capability} & \multirow{2}{*}{Remark} \\ \cline{3-5}
        & & Query Access & Target Query & Target Info. &  \\ \hline \hline
        \cite{dong2019efficient, zheng2021black, chen2020boosting} & \multirow{4}{*}{Adversarial Attack} & Decision & Chosen Pair by Adversary &\cellcolor{red!20}\red{Target Sample} &  N/A \\ 
        \cite{sharif2016accessorize, du2020sirenattack, chen2021real} &  & Score & \cellcolor{red!20}\red{Direct Query to Target Identity} & $\times$ & N/A \\ 
        \cite{kim2025non} &  & Score & Chosen Pair by Adversary & \cellcolor{red!20}\red{Target Sample} & N/A \\ 
        \cite{li2023sibling, jia2022adv, salar2025enhancing} &  & $\times$ & N/A & \cellcolor{red!20}\red{Target Sample} & Transferability \\ \hline
        \cite{mai2018reconstruction, duong2020vec2face, lu2021voxstructor, shahreza2024vulnerability} & \multirow{2}{*}{Reconstruction Attack} & \cellcolor{red!20}\red{Template} & N/A & \cellcolor{red!20}\red{Target Template} & N/A \\ 
        \cite{razzhigaev2021darker, vendrow2021realistic, jung2024face, kim2024scores} & & Score & \cellcolor{red!20}\red{Direct Query to Target Identity} & $\times$ & N/A \\  \hline
        \cite{damer2018morgan, colbois2023approximating} & Morphing Attack & $\times$ & N/A & \cellcolor{red!20}\red{Enrolled Samples} & N/A \\       
        \cite{nguyen2020generating, bontrager2018deepmasterprints, terhorst2022limited} & Wolf Attack & Score & \cellcolor{red!20}\red{Direct Query to Target Identity} & $\times$ & Transferability \\                 
        \cite{maiorana2014hill, galbally2010vulnerability, jeong2022analysis} & Impersonation Attack & Score & \cellcolor{red!20}\red{Direct Query to Target Identity} & $\times$ & N/A \\  
        \cite{khan2020mimicry, yoon2020new, kinnunen2019can} & Presentation Attack & $\times$ & N/A & \cellcolor{red!20}\red{Target Sample} & Direct Presentation \\
        \hline \hline
        Ours & Impersonation Attack & Score & Chosen Pair by Adversary & $\times$ & N/A\\ 
        \hline        
    \end{tabular}
    \label{tab:comp_table}
    \vspace{-5pt}
\end{table*}

==> texts/Backgrounds.tex <==
\subsubsection*{\bf Notation} 
For a set $\mathcal{X}$ and the metric function $d_{\mathcal{X}}: \mathcal{X} \times \mathcal{X} \rightarrow \mathbb{R}_{\ge 0}$, we denote $(\mathcal{X}, d_{\mathcal{X}})$ as the metric space. 
For a distribution $\mathcal{D}$, we denote $x \gets \mathcal{D}$ as the random sampling.
In particular, for a finite set $\mathcal{S}$, we denote $x \xleftarrow{\$} \mathcal{S}$ as the random uniform sampling over $\mathcal{S}$.

\subsubsection*{\bf Biometric Authentication Systems}
Let $\mathcal{B}$ be the set of biometrics and $(\mathcal{X}, d_{\mathcal{X}})$ be a metric space. 
We denote a function $F: \mathcal{B} \rightarrow \mathcal{X}$ as a \textit{feature extractor}.
In this context, we call each element of $\mathcal{X}$ a biometric template.
We expect that $F$ preserves the implicit similarity between biometric samples, i.e., biometric samples from the same identity are mapped to close templates, or vice versa.
With a feature extractor $F$, we define a biometric authentication system (BAS) as a pair of algorithms $(\mathsf{Enroll}, \mathsf{Auth})$ corresponding to enrollment and authentication, respectively.
Each algorithm has the following functionality:
\begin{itemize}
    \item $\mathsf{Enroll}$ takes a biometric sample $\mathfrak{v} \in \mathcal{B}$ and returns a corresponding template $t := \mathsf{Ext}(\mathfrak{v})$. Later, the BAS stores $t$ in its database.

    \item $\mathsf{Auth}$ takes a biometric sample $\mathfrak{v}' \in \mathcal{B}$ and the stored template $t$, returning a decision $0/1$ corresponding to ``reject" and ``accept". For a pre-determined threshold $\tau > 0$, this is typically implemented by $\mathds{1}(d_{\mathcal{X}}(\mathsf{Ext}(\mathfrak{v}'), t) < \tau)$.
\end{itemize}

For the ease of explanation, throughout this paper, we consider the BAS as a 1:1 verification system.
Our analysis can be naturally extended to a 1:N identification system, which will be discussed in Section~\ref{sec:extension}.


\subsubsection*{\bf False Match Rate and Impersonation Attack}
%
We briefly introduce false match rate (FMR) and a typical impersonation attack, which will serve as the background of our definition of adversarial FMR.
Informally, the FMR of the given BAS refers to the probability that a pair of biometrics from different identities is determined as the same identity.
Since the authentication algorithm is parametrized by the threshold $\tau$, so is FMR; a smaller $\tau$ gives a smaller FMR.
In standard benchmarks like IJB-C testsuite~\cite{maze2018iarpa}, FMR at the threshold $\tau$ is measured by $\mathsf{FMR}(\tau):= \frac{1}{|\mathcal{P}|}\sum_{(\mathfrak{v},\mathfrak{v}')\in \mathcal{P}} \mathds{1}(d_{\mathcal{X}}(\mathfrak{v}, \mathfrak{v}') < \tau)$, where $\mathcal{P}$ is the set of pairs of biometrics from different identities specified by the benchmark.

For the stored template $t$, we consider the impersonation attack as the problem of finding a biometric sample $\mathfrak{v}'$ such that $\mathsf{Auth}(\mathfrak{v}', t) = 1$, without knowing the stored template $t$.
The capability of the adversary depends on the attack scenarios; in usual real-world applications, the adversary does not know either the feature extractor of the target BAS or the enrolled biometrics.
In this setting, we can consider a simple impersonation attack that solely relies on FMR, so-called the \textit{zero-effort attack} mentioned in standards~\cite{grother2013biometric, iso2021iso19795}.
To impersonate the enrolled identity in the target BAS, the adversary selects one of the biometrics and tries to authenticate with this sample.
Provided that the threshold used for the benchmark dataset well represents the whole population, as commonly assumed in the standards~\cite{maze2018iarpa}, the adversary's attack success rate is the same as FMR.

